Riemannian Accelerated Zeroth-order Algorithm: Improved Robustness and Lower Query Complexity

Optimization problems with access to only zeroth-order information of the objective function on Riemannian manifolds arise in various applications, spanning from statistical learning to robot learning. While various zeroth-order algorithms have been proposed in Euclidean space, they are not inherently designed to handle the challenging constraints imposed by Riemannian manifolds. The proper adaptation of zeroth-order techniques to Riemannian manifolds remained unknown until the pioneering work of \cite{li2023stochastic}. However, zeroth-order algorithms are widely observed to converge slowly and be unstable in practice. To alleviate these issues, we propose a Riemannian accelerated zeroth-order algorithm with improved robustness. Regarding efficiency, our accelerated algorithm has the function query complexity of $\mathcal{O}(\epsilon^{-7/4}d)$ for finding an $\epsilon$-approximate first-order stationary point. By introducing a small perturbation, it exhibits a function query complexity of $\tilde{\mathcal{O}}(\epsilon^{-7/4}d)$ for seeking a second-order stationary point with a high probability, matching state-of-the-art result in Euclidean space. Moreover, we further establish the almost sure convergence in the asymptotic sense through the Stable Manifold Theorem. Regarding robustness, our algorithm requires larger smoothing parameters in the order of $\tilde{\mathcal{O}}(\epsilon^{7/8}d^{-1/2})$, improving the existing result by a factor of $\tilde{\mathcal{O}}(\epsilon^{3/4})$.

==> Estimators.tex <==
\section{Riemannian Coordinate-wise Zeroth-order Estimator}\label{sec.estimator}
% Traditionally, how to develop an efficient ZO gradient estimator attracts much attention. The two parameters $\mu$ and $m$ play crucial roles in balancing the tradeoff between approximation quality and computational costs. In Euclidean space, a classical ZO gradient estimator is the coordinate-wise gradient estimator (finite-difference gradient approximation) by taking $\{u_i\}$ as the standard basis of $\mathbb{R}^n$, thereby requiring $\Omega\left(n\right)$ function evaluations to obtain one gradient evaluation. An alternative approach for estimating gradients is using an arbitrary number of function value samples via choosing $\{u_i\}$ as random directions \cite{nesterov2017random,gao2018information}, such as Gaussian smoothing. Nevertheless, it remains unknown which of the deterministic or randomized schemes has an advantage when employed inside an optimization method until now \cite{scheinberg2022finite}.


% As mentioned in the introduction, the ZO gradient estimators in \cite{li2023stochastic, wang2021greene} can be seen as an extension of the randomized ZO gradient estimators on Euclidean space presented in \cite{nesterov2017random} and \cite{wang2021greene}, respectively. In addition to these randomized ZO gradient estimators, a more classical and traditional approach is the deterministic coordinate-wise ZO gradient estimator, also known as finite difference \cite{scheinberg2022finite}. As a complementary, we extend the coordinate ZO gradient estimator to Riemannian manifolds.


% Note that in the previous work \cite{li2023stochastic, wang2021greene, wang2023sharp}, Riemannian zeroth-order estimators are defined solely at each point $x \in \M$. Our definition extends to every point in the tangent space. Now we proceed to inspect the approximation quality of the estimator.
% \begin{lemma}\label{lemma.zero order estimator error}
%     Suppose that Assumption \ref{assum.lipschitz gradient} holds. Given a smoothing parameter $0 < \mu < b$, for any $(x, s_x) \in \T\M$ satisfying $\|s_x\| \in \mathbb{B}_{x, b-\mu}(0)$, it holds that
%     \begin{equation*}
%         \|g_x(s_x; \mu) - \nabla \hat f_x(s_x)\| \le \frac{l\mu\sqrt{d}}{2}.
%     \end{equation*}
% \end{lemma}
% \begin{proof}
%     From \autoref{assum:A3}, we obtain
%     \begin{subequations}
%         \begin{align}
%                 &\hat f_x(s+\mu e_i) - \hat f_x(s) \\
%             \le &\mu \inner{e_i}{\nabla \hat f_x(s)} + \frac{l}{2}\norm{\mu e_i}^2 \\
%             =   &\mu \inner{e_i}{\nabla \hat f_x(s)} + \frac{l\mu^2}{2},
%         \end{align}
%     \end{subequations}
%     and it further implies
%     \begin{subequations}
%         \begin{align}
%                 &\frac{\hat f_x(s+\mu e_i) - \hat f_x(s)}{\mu}e_i \\ 
%            \le  &\inner{e_i}{\nabla \hat f_x(s)} e_i + \frac{l\mu}{2}e_i
%         \end{align}
%     \end{subequations}
%     for all $i = 1, \ldots, d$. Therefore, we conclude
%     \begin{subequations}
%         \begin{align}
%                 &\|g^{\text{F}}_x(s; \mu) - \hat \nabla f_x(s)\| \\
%             =   &\|\sum_{i=1}^d \frac{\hat f_x(s+\mu e_i) - \hat f_x(s)}{\mu}e_i - \sum_{i=1}^d \inner{e_i}{\nabla \hat f_x(s)} e_i\| \\
%             \le &\frac{l\mu}{2}\|\sum_{i=1}^d e_i\| \\
%             =   &\frac{l\mu\sqrt{d}}{2},
%         \end{align}
%     \end{subequations}
%     where the last equality is due to the fact that $\{e_1, e_2, \ldots, e_d\}$ forms a standard basis. By a similar argument, we could validate the correctness of inequality \eqref{eq.error C}.
% \end{proof}
% \begin{lemma}
%     Given a smoothing parameter $0 < \mu < b$ and a pint $x \in \M$, for any $s \in \T_x\M$ satisfying $\|s\| \le b - \mu$, we have
%     \begin{equation*}
%         \|g^{\text{C}}_x(s; \mu) - \nabla \hat f_x(s)\| \le \frac{\rho\mu^2\sqrt{d}}{6}.
%     \end{equation*}
% \end{lemma}
% \begin{proof}
%     From \autoref{assum:A3}, we obtain
%     \begin{subequations}
%         \begin{align}
%                 &\hat f_x(s+\mu e_i) - \hat f_x(s) \\
%             \le &\mu \inner{e_i}{\nabla \hat f_x(s)} + \frac{\mu^2}{2}\inner{\nabla^2 \hat f_x(s) e_i}{e_i} + \frac{\rho}{6}\|\mu e_i\|^3 \\
%             =   &\mu \inner{e_i}{\nabla \hat f_x(s)} + \frac{\mu^2}{2}\inner{\nabla^2 \hat f_x(s) e_i}{e_i} + \frac{\rho\mu^3}{6}
%         \end{align}
%     \end{subequations}
%     and
%     \begin{subequations}
%         \begin{align}
%                 &\hat f_x(s-\mu e_i) - \hat f_x(s) \\
%             \le &-\mu \inner{e_i}{\nabla \hat f_x(s)} + \frac{\mu^2}{2}\inner{\nabla^2 \hat f_x(s) e_i}{e_i} + \frac{\rho\mu^3}{6}.
%         \end{align}
%     \end{subequations}
%     Consequently, we see
%     \begin{subequations}
%         \begin{align}
%             &\hat f_x(s+\mu e_i) - \hat f_x(s-\mu e_i) - 2\inner{e_i}{\nabla \hat f_x(s)} \\
%             =   &(\hat f_x(s+\mu e_i) - \hat f_x(s) - \mu \inner{e_i}{\nabla \hat f_x(s)} + \frac{\mu^2}{2}\inner{\nabla^2 \hat f_x(s) e_i}{e_i}) \\
%             -   &(\hat f_x(s-\mu e_i) - \hat f_x(s) + \mu \inner{e_i}{\nabla \hat f_x(s)} + \frac{\mu^2}{2}\inner{\nabla^2 \hat f_x(s) e_i}{e_i}) \\
%             \le &\frac{\rho\mu^3}{3},
%         \end{align}
%     \end{subequations}
%     and it follows
%     \begin{subequations}
%         \begin{align}
%             &\|g^{\text{C}}_x(s; \mu) - \hat \nabla f_x(s)\| \\
%             =   &\|\sum_{i=1}^d \frac{\hat f_x(s+\mu e_i) - \hat f_x(s-\mu e_i)}{2\mu}e_i - \sum_{i=1}^d \inner{e_i}{\nabla \hat f_x(s)} e_i\| \\
%             \le &\frac{\rho\mu^2}{6}\|\sum_{i=1}^d e_i\| \\
%             =   &\frac{\rho\mu^2\sqrt{d}}{6}.
%         \end{align}
%     \end{subequations}
% \end{proof}

% From Lemma \ref{lemma.zero order estimator error}, the update at Line 4 in Algorithm \ref{alg.ZGD} can be viewed as an inexact Riemannian gradient descent, and thus the key ingredient is to check the function value decrease in each iterate when 

% To analyze the iteration complexity of Algorithm \ref{alg.ZGD}, we select an appropriate value of the smoothing parameter $\mu$ to balance the approximation error of the zeroth-order gradient estimator in Lemma \ref{lemma.zero order estimator error} and the decrease in function value at each iteration. 


